The Effect of Weather Conditions on Fertilizer Applications: A Spatial Dynamic Panel Data Analysis

Given the extreme dependence of agriculture on weather conditions, this paper analyses the effect of climatic variations on this economic sector, by considering both a huge dataset and a flexible spatio-temporal model specification. In particular, we study the response of N-fertilizer application to abnormal weather conditions, while accounting for other relevant control variables. The dataset consists of gridded data spanning over 21 years (1993-2013), while the methodological strategy makes use of a spatial dynamic panel data (SDPD) model that accounts for both space and time fixed effects, besides dealing with both space and time dependences. Time-invariant short and long term effects, as well as time-varying marginal effects are also properly defined, revealing interesting results on the impact of both GDP and weather conditions on fertilizer utilizations. The analysis considers four macro-regions -- Europe, South America, South-East Asia and Africa -- to allow for comparisons among different socio-economic societies. In addition to finding both spatial (in the form of knowledge spillover effects) and temporal dependences as well as a good support for the existence of an environmental Kuznets curve for fertilizer application, the paper shows peculiar responses of N-fertilization to deviations from normal weather conditions of moisture for each selected region, calling for ad hoc policy interventions.

==> MyDef/def_color.tex <==
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% COLORS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\definecolor{darkross}{rgb}{0.008,0.412,0.471}
\definecolor{middleross}{rgb}{0.012,0.580,0.663}
\definecolor{lightross}{rgb}{0.016,0.749,0.855}
\definecolor{darkblue}{rgb}{0.067,0.008,0.471}
\definecolor{middleblue}{rgb}{0.094,0.012,0.663}
\definecolor{lightblue}{rgb}{0.122,0.016,0.855}
\definecolor{darkpurple}{rgb}{0.471,0.008,0.412}
\definecolor{middlepurple}{rgb}{0.663,0.012,0.580}
\definecolor{lightpurple}{rgb}{0.855,0.016,0.749}
\definecolor{darkbrown}{rgb}{0.471,0.067,0.008}
\definecolor{middlebrown}{rgb}{0.663,0.094,0.012}
\definecolor{lightbrown}{rgb}{0.855,0.122,0.016}
\definecolor{darkolive}{rgb}{0.412,0.471,0.008}
\definecolor{middleolive}{rgb}{0.580,0.663,0.012}
\definecolor{lightolive}{rgb}{0.749,0.855,0.016}
\definecolor{darkgreen}{rgb}{0.008,0.417,0.067}
\definecolor{middlegreen}{rgb}{0.012,0.663,0.094}
\definecolor{lightgreen}{rgb}{0.016,0.855,0.122}
\definecolor{darkocre}{rgb}{0.471,0.298,0.008}
\definecolor{middleocre}{rgb}{0.663,0.420,0.012}
\definecolor{lightocre}{rgb}{0.855,0.541,0.016}
%
\def\colorred{\color{red}}
\def\colorblue{\color{middleblue}}
\def\colorgreen{\color{green}}
\def\coloryellow{\color{yellow}}

\def\colordarkross{\color{darkross}}
\def\colordarkblue{\color{darkblue}}
\def\colorlightblue{\color{lightblue}}
\def\colorlightbrown{\color{lightbrown}}
\def\colordarkgreen{\color{darkgreen}}

==> MyDef/def_letters_acc.tex <==
\def\ac{\`a}
\def\ec{\`e}
\def\uc{\`u}
\def\oc{\`o}

\def\acsp{\`a }
\def\ecsp{\`e }
\def\ucsp{\`u }
\def\ocsp{\`o }

\def\qmo{``}
\def\qmc{''}
\def\qmcsp{'' }


